Guarding Polyominoes Under $k$-Hop Visibility

We study the Art Gallery Problem under $k$-hop visibility in polyominoes. In this visibility model, two unit squares of a polyomino can see each other if and only if the shortest path between the respective vertices in the dual graph of the polyomino has length at most $k$. In this paper, we show that the VC dimension of this problem is $3$ in simple polyominoes, and $4$ in polyominoes with holes. Furthermore, we provide a reduction from Planar Monotone 3Sat, thereby showing that the problem is NP-complete even in thin polyominoes (i.e., polyominoes that do not a contain a $2\times 2$ block of cells). Complementarily, we present a linear-time $4$-approximation algorithm for simple $2$-thin polyominoes (which do not contain a $3\times 3$ block of cells) for all $k\in \mathbb{N}$.

==> arxiv--conclusion.tex <==
In this paper, we investigated a covering problem motivated by the placement of carsharing stations within a city, and a maximum walking range of customers; we called it the \textsc{Minimum $k$-Hop Guarding Problem in Polyominoes}. 
In particular, our guards can see every square within a hop distance of $k$, resulting in guards that can ``see'' around (many) corners. 
We showed that the problem is \NP-complete even in $1$-thin polyominoes with holes for $k\geq 2$, i.e., polyominoes that do not contain a $2\times 2$~block of unit squares.
Furthermore, we studied the VC dimension of the problem in both simple polyominoes and polyominoes with holes, and presented tight bounds in both cases: it is $3$ in simple polyominoes, and $4$ in polyominoes with holes.
We further gave a linear-time $4$-approximation algorithm for simple $2$-thin polyominoes.

In our opinion, the most interesting open questions are:
(1)~Is there a more general approximation framework for arbitrary $k$ in arbitrary simple polyominoes?
(2)~Is there a constant-factor approximation for polyominoes with holes?
(3)~Imagine that the city center requires a higher density of carsharing stations, while longer distances are accepted in the peripheral areas;
What can be said about the problem if it is allowed to place various classes of guards having different values of $k$?
